Lectures on the Routh-Hurwitz problem

The notes contain a streamlined account on stability of univariate polynomials and related problems

==> MACRO2_en.tex <==
%%% 22 Jan 2004
%%% Макросы для 2-й части методического пособия
%%% "Проблема Рауса-Гурвица"

\theoremstyle{plain}
\newtheorem{thm}{Теорема}[section]
\newtheorem*{res}{Теорема}
\newtheorem{cor}{Следствие}[section]
\newtheorem{lem}{Лемма}[section]
\newtheorem{problem}{Задача}[section]

\renewcommand{\proofname}{Доказательство}

\theoremstyle{definition}
\newtheorem{defn}{Определение}[section]
\newtheorem{note}{Замечание}[section]

\DeclareMathOperator{\CMD}{ОНД}
\DeclareMathOperator{\CMM}{ОНК}

\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\PR}{P\mathbb R}
\DeclareMathOperator{\sgn}{sign}
\DeclareMathOperator{\ran}{rank}
\DeclareMathOperator{\Pos}{pos}
\DeclareMathOperator{\Neg}{neg}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Res}{Res}

%\newcommand{\R}{\mathbb R}
%\newcommand{\C}{\mathbb C}

\newcommand{\IndI}{\Ind_\infty}
\newcommand{\IndC}{\Ind_{-\infty}^{+\infty}}
\newcommand{\IndPR}{\Ind_{\PR}}

\newcommand\SL{\pmb{S}\pmb{L}(2,\mathbb{R})}

\newcommand\thr{}
\newcommand\tvr{}

\let\phi\varphi
\let\epsilon\varepsilon
\let\kappa\varkappa
\let\leq\leqslant
\let\geq\geqslant

